Engaging Millennials into Learning Formal Methods

This paper summarizes our experience in teaching courses on formal methods (FM) to Computer Science (CS) and Software Engineering (SE) students at various universities around the world, including University of Madeira (UMa) in Portugal, Pontificia Universidad Javeriana (PUJ) and University of Los Andes (Uniandes) in Colombia, Carnegie Mellon University (CMU) in the USA, and at Innopolis University (INNO) in the Russian Federation. We report challenges faced during the past 10 to 15 years to teach FM to millennials undergradu- ate and graduate students and describe how we have coped with those challenges. We formulate a characterization of millennials, based on our experience, and show how this characterization has shaped our decisions in terms of course structure and content. We show how these decisions are reflected on the current structure of the MSS (Models of Software Systems) course that currently runs as part of the MSIT-SE (Master of Science in Information Technology - Software Engineering) programme offered at INNO. We have conducted two surveys among students, the first one at CMU and the second one at INNO that we have used to document and justify our decisions. The first survey is about the choice of Event-B as mathematical formalism and the second one is about the organization of teams of students within the classroom to work on software projects based on Event-B.

==> puj.tex <==
\section{Formal Methods at Pontificia Universidad Javeriana}
\label{sec:puj}

Engineering in Computer Science (CS) at Pontificia Universidad Javeriana
(PUJ) is a 5 years programme, structured per semesters, comprising a 2
years common trunk in physics and mathematics, shared by all other
engineering programs, including 2 courses in discrete mathematics and
logic. This common trunk is followed by a 3 years programme in CS,
with about a 30$\%$ course charge in economics and humanities. The
discrete mathematics, as well as all the basic computer related
courses comply with the ACM/IEEE undergraduate CS 
curriculum (\texttt{http://\-sites.\-computer.\-org/\-ccse/}). There
are two basic courses in Software Engineering (SE):

\begin{enumerate}
\item Software processes dealing with fundamental design principles,
  API design, tool design, software life cycles and capability
  models.

\item Software Engineering and management, dealing with software
  requirements specifications (SRS), project management, validation
  and verification, and software evolution.
\end{enumerate}

These courses are scheduled for sixth and the seventh semester
undergraduate students respectively. A formal software development
course is given in the sixth semester, at the same time as the
software processes course. Additionally, there is a case-based SE
workshop scheduled for eighth semester students. Topics for this
workshop vary, yet it has often been the case that the workshop has
been dedicated to software verification with JML.

Formal modeling courses are not part of the core in the ACM/IEEE
curriculum. PUJ decided to include formal modeling courses into the SE
programme mainly for two reasons:
$(i.)$ a survey among recruiting executives of companies in the city of Cali 
revealed that they consider the ability to clearly reason about a software
design as a key (usually lacking) competence in young professionals,
and $(ii.$) the economic development plan of Cali pointed at software
production as a key strategy and increasing software quality as the
most pressing need in this realm.

PUJ's CS department keeps a close relations with ParqueSoft, the
biggest Colombian technological cluster, with more than 200 software
companies and 800 software developers
(\texttt{http://\-www.\-par\-que\-soft.\-com}). ParqueSoft software
companies are typically launched by students from the three biggest
universities in Cali. ParqueSoft's total sales are about US $\$$47
million a year. About half of these companies have achieved standard
quality assurance certifications. Most CS students at
PUJ conduct internships in these and
other companies based in Cali during their third year of
studies. PUJ's CS department
encourages students to initiate software start-ups at ParqueSoft
through an entrepreneurship joint educational program. Students in
this program substitute their engineering degree final thesis report
with a technical report on their proposed software venture.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model-driven Software Engineering with Event-B}
\label{subsec:mdeb}

This course illustrates the advantages of using formal techniques for
modelling systems and developing software. It puts forward the idea of
using formal techniques as guiding principles for thinking a system
model from scratch in a disciplined way.  This Event-B course follows
what J.-R.Abrial calls ``the parachute strategy'', in which systems
are first considered from a very abstract and simple point of view,
with broad fundamental observations. This view usually comprises few
simple invariant properties that students can easily grasp,
\textit{e.g.}, defining what can reasonably be expected from the
operation of such a system. \emph{Liveness} properties
\cite{PnueliLTL77} are also introduced at this level. Once students
understand the system completely, they are asked to develop small
variants of it and to discharge all the Proof Obligations (POs). The second step
is to consider a refinement by adding a viewpoint observation in such
a way that the new model keeps a palpable behavioural relation with
its abstraction. Students are then encouraged to find by themselves
precise relationships between abstract and concrete variables that
guarantee coherent behaviour between both models.

As more experience is gained in the modelling framework, development
of more complete systems comprising several refinements is
attempted. In these refinements, the way how invariant properties can
be used as a tool for tuning events is stressed. Systems that are very
familiar to students, such as a soccer match, are used at this stage
for them to be able to develop an intuitive, yet precise, idea of the
use of refinement conditions. In the final stage of the course, a
model of a more real-life system is constructed, alternating designs
discussed in class with refinements supplied by students in their
homework.

Although a broad review of first order logic and set theory is given
at the beginning of the course, our strategy is to introduce Event-B
modelling language constructs, such as relations, functions, sets and
their operations as they are needed to express some specific property
of the system at hand. Even the review of mathematical logic is done
in a very instrumental way, stressing its use in modelling. Students
are never required to do by-hand formal proofs of any logic formula,
but they are constantly encouraged to argue about its validity. The
idea behind this is to help students build a more ``friendly''
attitude towards mathematical formalisms, by showing them how a
machine can do the tedious job of proving a formula in their place.

This course uses the Rodin platform intensively
(\url{http://wiki.event-b.org/index.php/Rodin\_Platform}). This
platform comprises an intuitive graphical interface based on Eclipse
(\url{http://www.eclipse.org}) in which users can edit, prove
and animate an Event-B model. In the beginning of the course, students
are required to edit and type-check models in Rodin, though, instead
of proving them, the animator plug-in is used to understand the model
behaviour. In any case, initial models are chosen so that Rodin can
automatically prove them. As familiarity with the tool increases, the
models considered have a few POs that Rodin cannot prove
automatically. At this point, the Mathematical Language chapter of
the Rodin manual \cite{RodinD7} is presented. This provides a 
intuitive, yet rigorous, introduction to propositional and predicate
logic from the vantage point of carrying out automatic proofs in those
systems. Students can then understand Rodin proof strategies, and also
relate this knowledge to how they can better guide Rodin's interactive
prover. From this point on, students are required to fully prove their
developments with Rodin.

The second part of the course uses Event-B to construct programs (as
opposed to systems). This is done in Event-B by considering an
abstract system that just specifies preconditions (context part and
invariants) having an event computing in one step the result of the
program (i.e. specifying its post-condition). Refinements of this
initial model proceed just as for system models. The last refinement
is such that each event could easily be coded in some imperative
programming language. Rules to automatically translate this last
refinement into code can be easily devised but, unfortunately, as of
this writing they have not been integrated into Rodin so that students
must do this by hand.

The final part of the course deals with software systems. These, in
principle, could be modelled in Event-B just as any other system. In
our view, however, the lack of constructs to relate machines in
different ways (e.g. as provided by Z~\cite{SpiveyIntro2Z}) makes its
use problematic in a pedagogical sense. The point is that students
are, in other courses and in their initial job experiences, used to
build software out of software pieces already available. 

\subsection{Experience with the Course}
\label{SecExpB}
The course is scheduled in the sixth semester, when students have
already taken courses in programming, object oriented design and
database models. Students who attend the course have already learnt to
build software in a different way what they are taught during the
Event-B course. This creates skepticism among students from the very
beginning of the course, which makes it difficult to keep the
necessary motivation alive. We 
use two strategies to tackle this problem. First, systems considered
at the beginning of the course pertain to situations that are familiar
to students, yet not trivial. Second, in the software development
part, students are required to constantly assess advantages and
disadvantages of the same problem modelled with Event-B and with the
traditional methodologies used in other courses. Nevertheless, we have
found that for this purpose a transition going from traditional ways
of thinking systems to JML and then to Event-B greatly diminishes the
initial skepticism and, at the same time, helps students to place each
methodology in the right context of application.

A second issue is the use of mathematical formalisms. Students are
evermore demanding to see clear relationships between their future
professional activity and the mathematics they are being taught. In
the first offerings of this course, mathematical formalisms were given
a central role from the outset and thus all logic and mathematics
needed to express Event-B POs and constructs was
presented at the beginning of the course. This only aggravated the
motivational problem. Current versions of the course, as stated above,
develops mathematical constructs along the course, always with a clear
view of what precisely they are intended for in the problem at
hand. Moreover, students are required to express in their own words
those fundamental properties of a system, prior to their formalisation
using the mathematical language of Event-B.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

